Exploring the nature of Galactic unassociated sources detected by the Fermi-LAT

We investigate the nature of the unassociated sources detected by the Fermi-LAT close (|b|<10{\deg}) to the Galactic plane, representing 16% of all sources in the 4FGL-DR4 catalog. The bulk of these sources (referred to as soft Galactic unassociated sources, SGUs) exhibit properties not found in known classes of gamma-ray emitters, as confirmed by a machine-learning classification approach. In particular, these properties include a steep, curved spectrum peaking below 1 GeV and a specific Galactic-latitude distribution with both a narrow and a broad component (dubbed the spike and the shoulder, respectively). Some source clusters are highlighted. New plausible source classes are explored, but only star-forming regions are found to account for a significant fraction (at most 10%) of the unassociated population. A thorough search for counterparts to the 175 brightest sources brings out a number of plausible counterparts but does not reveal clues about the nature of the whole population. We investigate the possibility that SGUs originate from mismodeled clumps of diffuse emission. Using Monte Carlo simulations, the SGU spectra can be reproduced in this scenario under an ad hoc condition concerning the clump spatial extension. The possible connection between the SGUs and gas not accounted for by the 12CO tracer is explored using the 13CO MOPRA data but leads to inconclusive results. The origin of SGUs being related to diffuse emission remains plausible. However, a scenario whereby SGUs represent a new class of gamma-ray emitters cannot be fully excluded.

==> GUs_wo_count_paper.tex <==
4FGL J0009.2+6847 & 
4FGL J0204.7+6656 & 
4FGL J0754.9-3953 & 
4FGL J0826.1-5053 & 
4FGL J0828.4-4444 & 
4FGL J0853.6-4306 & 
4FGL J1026.2-5731 & 
4FGL J1208.0-6900 & 
4FGL J1220.1-5558 & 
4FGL J1244.3-6233 & 
4FGL J1404.8-5237 & 
4FGL J1412.1-6631 & 
4FGL J1534.0-5232 & 
4FGL J1538.0-4638 & 
4FGL J1548.1-4416 & 
4FGL J1603.3-6010 & 
4FGL J1620.8-4958c & 
4FGL J1640.3-4917 & 
4FGL J1643.3-3148 & 
4FGL J1704.8-4030 & 
4FGL J1725.1-1924 & 
4FGL J1729.1-3503 &  
4FGL J1743.7-4321 & 
4FGL J1744.0-1311 & 
4FGL J1744.7-1557 & 
4FGL J1748.3-2906 & 
4FGL J1754.6-2933 & 
4FGL J1758.7-4109 & 
4FGL J1805.1-3618 & 
4FGL J1812.8-3144 & 
4FGL J1815.8-1416 & 
4FGL J1817.9-3334 & 
4FGL J1818.6-3206 & 
4FGL J1819.9-1530 & 
4FGL J1819.9-2926 & 
4FGL J1830.7-1634 & 
4FGL J1830.8-3132 & 
4FGL J1840.4-1139 & 
4FGL J1843.3-1242 & 
4FGL J1852.6+0203 & 
4FGL J1857.1+0056 & 
4FGL J1901.8-0718 & 
4FGL J1902.5+0654 & 
4FGL J1906.1+1651 & 
4FGL J1912.5+1320 & 
4FGL J1926.4+1602 &  
4FGL J1931.1+1656 & 
4FGL J1944.8+4301 & 
4FGL J1948.9+3414 & 
4FGL J2027.0+2811 &  
4FGL J2108.0+5155 & 
4FGL J2114.3+5023 & 
4FGL J2116.2+3701 & 
4FGL J2117.9+3729 & 
4FGL J2218.8+4736 & 
4FGL J2220.8+6319 & 

